ICRC 2023 Gamma-ray Rapporteur Talk: a quick walk through the gamma-ray universe

This document attempts to summarize the Gamma ray section of the 38th International Cosmic Ray Conference held in Nagoya. There were 387 contributions submitted to this section distributed in 22 parallel oral and three poster sessions, plus four related highlight or review talks. The information included in this contribution is a description of what was reported at the conference, that represent the state of the art of the field.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

